From optimal score matching to optimal sampling

The recent, impressive advances in algorithmic generation of high-fidelity image, audio, and video are largely due to great successes in score-based diffusion models. A key implementing step is score matching, that is, the estimation of the score function of the forward diffusion process from training data. As shown in earlier literature, the total variation distance between the law of a sample generated from the trained diffusion model and the ground truth distribution can be controlled by the score matching risk. Despite the widespread use of score-based diffusion models, basic theoretical questions concerning exact optimal statistical rates for score estimation and its application to density estimation remain open. We establish the sharp minimax rate of score estimation for smooth, compactly supported densities. Formally, given \(n\) i.i.d. samples from an unknown \(\alpha\)-H\"{o}lder density \(f\) supported on \([-1, 1]\), we prove the minimax rate of estimating the score function of the diffused distribution \(f * \mathcal{N}(0, t)\) with respect to the score matching loss is \(\frac{1}{nt^2} \wedge \frac{1}{nt^{3/2}} \wedge (t^{\alpha-1} + n^{-2(\alpha-1)/(2\alpha+1)})\) for all \(\alpha > 0\) and \(t \ge 0\). As a consequence, it is shown the law \(\hat{f}\) of a sample generated from the diffusion model achieves the sharp minimax rate \(\bE(\dTV(\hat{f}, f)^2) \lesssim n^{-2\alpha/(2\alpha+1)}\) for all \(\alpha > 0\) without any extraneous logarithmic terms which are prevalent in the literature, and without the need for early stopping which has been required for all existing procedures to the best of our knowledge.

==> upper/sk_edit_upper_bound_text.tex <==
For score estimation with respect to the score matching loss (\ref{def:score_matching_loss}), we establish the following minimax upper bound for any H\"{o}lder exponent $\alpha > 0$ and time $0 < t \lesssim 1$. 
\begin{theorem}
\label{thm:score_upperbound}
For $\alpha > 0 $, there exist universal constants $c_1 = c_1(\alpha, L)$ and $c_2 = c_2(\alpha, L)$ only dependent on $\alpha$ and $L$ such that
\begin{equation*}
\inf_{\hat{s}} \sup_{f \in \mathcal{F}_\alpha} \bE\left(\int_{-\infty}^{\infty} \left|\hat{s}(x, t) - s(x, t)\right|^2 \, p(x, t) \,\rd x \right) \le c_1\left(\frac{1}{nt^{3/2}} \wedge \left(n^{-\frac{2(\alpha-1)}{2\alpha+1}} + t^{\alpha-1}\right)\right)
\end{equation*}
for all $0 < t < c_2$. 
\end{theorem}

To describe our methodology, first note the score function can be written as $s(x,t)=\frac{\psi(x,t)}{p(x,t)} = \frac{(\phi_t' * f)(x)}{(\phi_t * f)(x)}$ where $\psi(x,t) = \frac{\partial}{\partial x} p(x,t)$ is the density derivative. At a high level, \(\psi\) and \(p\) will be estimated by separate estimators, which will later be combined into a score estimator. We employ different methodology depending on whether the noise level \(t\) is high or low. Throughout this section, denote the available data as \(\mu_1,...,\mu_n \overset{iid}{\sim} f\).  

\subsection{High-noise regime}
In the high-noise regime \(t \gtrsim n^{-\frac{2}{2\alpha+1}}\), a direct idea for constructing a score estimator is to consider unbiased estimators of both the density derivative $\psi(x,t)$ and the density $p(x,t)$. The unbiased estimators $\hat{\psi}_n(x,t)$ and $\hat{p}_n(x,t)$ can be obtained by replacing $f$ in \(\psi\) and \(p\) with the empirical distribution $\frac1n\sum_{j=1}^n \delta_{\mu_j}$, 
\[\hat{\psi}_n(x, t) = \frac1n \sum_{j=1}^n \phi_t'(x-\mu_j), ~~~\hat{p}_n(x, t) = \frac1n \sum_{j=1}^n \phi_t(x-\mu_j). \]
The natural score estimator is \(\frac{\hat{\psi}_n(x, t)}{\hat{p}_n(x, t)}\). The individual mean integrated squared errors (MISE) only contain the variance terms and can be upper bounded as
\begin{equation}
\label{eqn:intro-1}
\bE \int_{-\infty}^{\infty} \left|\hat{\psi}_n(x, t) - \psi(x,t)\right|^2 \,\rd x \lesssim \frac{1}{nt^{3/2}}, ~~~\bE \int_{-\infty}^{\infty} \left|\hat{p}_n(x, t) - p(x,t)\right|^2 \,\rd x \lesssim \frac{1}{nt^{1/2}}
\end{equation}
through a simple calculation. However, bounding the score matching loss (\ref{def:score_matching_loss}) is not straightforward since $p(x,t)$ and $\hat{p}_n(x,t)$ both can be exponentially small when $|x|$ is sufficiently large, which is problematic since they appear in the denominators of \(s\) and the natural score estimator respectively. To overcome this technical obstacle, a regularization trick is widely applied in various existing works to yield the score estimator $\hat{s}_n(x,t) = \frac{\hat{\psi}_n(x,t)}{\hat{p}_n(x,t)\vee \varepsilon}$, where the regularization $\varepsilon = n^{-2}$ is typically chosen (e.g. \cite{wibisono_optimal_2024}). Through this regularization, Wibisono et al. \cite{wibisono_optimal_2024} further control the score matching risk by the Hellinger distance but incur additional $\poly(\log n)$ factors. To avoid these logarithmic terms, we employ a regularizer which is a function of $x$ instead of one which is constant in $x$. Specifically, we use
\begin{equation*}
    \hat{s}_n(x,t) = \frac{\hat{\psi}_n(x,t)}{\hat{p}_n(x,t)\vee \varepsilon(x)}
\end{equation*}
with the choice $\varepsilon(x) := c_d\int_{-1}^1 \phi_t(x-\mu) \,\rd \mu $. Notice $\varepsilon(x) \le p(x,t) \le C_d / c_d \cdot \varepsilon(x)$ always holds for \(f \in \mathcal{F}_\alpha\). Consequently, the score matching risk can be split into two separate errors corresponding to the density and its derivative,
\begin{equation}\label{eqn:score_loss_deconstruct}
\bE \int_{-\infty}^{\infty} \left(\hat{s}_n(x,t)-s(x,t)\right)^2 \, p(x,t) \,\rd x \lesssim \int_{\infty}^{\infty} \frac{\bE (\hat{\psi}_n(x, t)-\psi(x,t))^2}{p(x,t)} + s(x,t)^2 \frac{\bE (\hat{p}_n(x, t)-p(x,t))^2}{p(x,t)} \,\rd x.
\end{equation}
To bound the error, we consider three different regions: the internal part $D_1 = \{x:~|x|<1-\sqrt{Ct\log(1/t)}\}$, the boundary part $D_2 = \{x:~1-\sqrt{Ct\log(1/t)} \le |x| \le 1+C\sqrt{t}\}$ and the external part $D_3 = \{x:~|x| > 1+C\sqrt{t}\}$. First consider that for \(x \in D_1 \cup D_2\) we have $p(x,t)\gtrsim 1$. It can be further shown $|s(x,t)|\lesssim \frac{1}{\sqrt{t}}$. Therefore, it is clear from (\ref{eqn:score_loss_deconstruct}) that the score matching risk is upper bounded by \(\frac{1}{nt^{3/2}}\) when the integral is taken only over \(D_1 \cup D_2\) instead of \(\R\); the difficulty of estimating the derivative \(\psi\) dominates. 

For the external part $D_3$, we compare the exponential decay rates of the numerators and denominators and show that the integrand in (\ref{eqn:score_loss_deconstruct}) itself exhibits exponential decay and thus yields a risk which is dominated by \(\frac{1}{nt^{3/2}}\). Therefore, \(\hat{s}_n\) constructed from these unbiased estimators furnishes the minimax upper bound, 
\[\sup_{f \in \mathcal{F}_\alpha} \bE\left(\int_{-\infty}^{\infty} \left|\hat{s}_n(x, t) - s(x, t)\right|^2 \, p(x, t) \,\rd x \right) \lesssim \frac{1}{nt^{3/2}}.\]
The result is far from satisfactory because the bound diverges as the noise level $t\rightarrow 0$. A naive application of (\ref{eqn:dtv_score_bound}), even with early stopping incorporated, will yield a suboptimal convergence rate instead of the sharp \(n^{-\frac{2\alpha}{2\alpha+1}}\) scaling. Indeed, this is the essence of the shared shortcomings of existing works \cite{oko_diffusion_2023,block_generative_2022,wibisono_optimal_2024,zhang_minimax_2024}. 

\subsection{Low-noise regime}
In the low-noise regime \(t \lesssim n^{-\frac{2}{2\alpha+1}}\) with \(\alpha \ge 1\), the optimal rate is \(n^{-\frac{2(\alpha-1)}{2\alpha+1}}\) as seen in (\ref{eqn:rate}). To achieve this rate, we develop a kernel-based score estimator. As before, the derivative \(\psi\) and the density \(p\) are separately estimated, but now the smoothness of \(f\) is explicitly exploited by way of kernel smoothing. According to [Cite XXX], there exists a kernel density estimator \(\hat{f}\) of the data generating density $f$ such that
\[\bE \left(\hat{f}^{(k)}(x) - f^{(k)}(x)\right)^2\lesssim n^{-\frac{2(\alpha-k)}{2\alpha+1}},~~~k=0,1,\ldots, \lfloor\alpha\rfloor\]
for $x\in [-1, 1]$. The score estimator is inspired by the direct plugin of $\hat{f}$, with some regularization applied. When $x$ lies in the internal part (i.e. $D_1$), we still apply the regularizer $\varepsilon(x)$ proposed in the high-noise regime, 
\[\hat{s}(x,t) = \frac{\hat{\psi}(x,t)}{\hat{p}(x,t) \vee \varepsilon(x)}.\]
For the internal case where $x\in D_1$, the proof is very similar to the high-noise regime and the upper bound $n^{-\frac{2(\alpha-1)}{2\alpha+1}}$ can be easily obtained since the density derivative estimation error dominates the other terms. 

However, when $x$ lies in the boundary and external parts (i.e $D_2 \cup D_3$), a component-wise lower bound regularizer is required. We construct
\[\hat{s}(x,t) = \frac{(\phi_t'* \hat{f})(x)}{(\phi_t * \widetilde{f})(x)}\]
where $\widetilde{f} = \hat{f} \vee \frac{c_d}{2}$. In order to establish the optimal convergence rate for the boundary and external cases, we directly operate  
\begin{equation}
\label{eqn:intro-2}
\hat{s}(x,t)-s(x,t) = \frac{(\phi_t'* \widetilde{f})(x)\cdot\left(\phi_t * f\right)(x) - (\phi_t * \widetilde{f})(x)\cdot\left(\phi_t'* f\right)(x)}{(\phi_t * \widetilde{f})(x)\cdot \left(\phi_t * f\right)(x)}
\end{equation}
instead of splitting as in (\ref{eqn:score_loss_deconstruct}). 

For \(x \in D_2\), the denominator in (\ref{eqn:intro-2}) is lower bounded by a constant, and so it suffices to focus on the numerator. In other words, letting \(J(x, t)\) denote the numerator in (\ref{eqn:intro-2}), it suffices to show \(\int_{D_2} \bE(J(x, t)^2) \, \rd x \lesssim n^{-\frac{2(\alpha-1)}{2\alpha+1}}\). For the kernel-based density estimator $\hat{f}$, we have $\|\hat{f}-f\|_\infty < \frac{c_d}{2}$, which leads to $\widetilde{f}=\hat{f}$ except on an event of exponentially small probability. Working on the high-probability event \(\{\widetilde{f} = \hat{f}\}\), observe that integration by parts yields 
\begin{align*}
    (\varphi_t' * f)(x) &= \varphi_t(x+1)f(-1) - \varphi_t(x-1)f(1) + \int_{-1}^{1} \varphi_t(x-\mu) f'(\mu) \,\rd \mu, \\
    (\varphi_t' * \tilde{f})(x) &= \varphi_t(x+1)\hat{f}(-1) - \varphi_t(x-1)\hat{f}(1) + \int_{-1}^{1} \varphi_t(x-\mu)\hat{f}'(\mu) \, \rd \mu. 
\end{align*}
Therefore, we have the bound \(\bE(J(x, t)^2) \lesssim \bE (J_1(x, t)) + \bE (J_2(x, t)) + \bE (J_3(x, t))\) where 
\begin{align*}
    J_1(x, t) &= |\varphi_t(x-1)|^2|f(1) (\varphi_t * \hat{f})(x) - \hat{f}(1) (\varphi_t * f)(x)|^2, \\
    J_2(x, t) &= |\varphi_t(x+1)|^2 |f(-1)(\varphi_t * \hat{f})(x) - \hat{f}(-1) (\varphi_t * f)(x)|^2, \\
    J_3(x, t) &= \left((\varphi_t * f)(x) \int_{-1}^{1} \varphi_t(x-\mu) \hat{f}'(\mu) \,\rd \mu - (\varphi_t * \hat{f})(x)\int_{-1}^{1} \varphi_t(x-\mu) f'(\mu)\, \rd\mu\right)^2.
\end{align*}
Without loss of generality, suppose \(x \in D_2\) is positive (an analogous argument applies for negative \(x\)). Then by definition of \(D_2\), we have \(|x-1| < \sqrt{Ct\log(1/t)}\) and so \(J_2\) can be shown to be exponentially small and thus negligible. Unsurprisingly, \(J_3\) can also be bounded in a straightforward way to obtain the desired \(n^{-\frac{2(\alpha-1)}{2\alpha+1}}\) rate since we have already passed to the derivatives of \(f\) and \(\hat{f}\). 

The worrisome term is \(J_1\), whose existence is due to the discontinuity of \(f\) and \(\hat{f}\) at the point \(1\). As pointed out in Remark \ref{remark:boundary}, the expert reader might expect the discontinuity to cause some slowdown in the rate. Specifically, one might expect that \(\hat{f}(1)\) can not estimate \(f(1)\) at a (squared) rate faster than \(n^{-\frac{2\alpha}{2\alpha+1}}\), and so it might be hopeless to improve upon the bound \(\bE(J_1(x, t)) \lesssim \frac{1}{t} \cdot n^{-\frac{2\alpha}{2\alpha+1}}\). This bound is not quite good enough since it would only deliver \(\int_{D_2 \cap \R^+} \bE \left(J_1(x, t)\right) \, \rd x \lesssim n^{-\frac{2\alpha}{2\alpha+1}} \cdot \sqrt{\frac{\log(1/t)}{t}}\), which is larger than the bound \(n^{-\frac{2(\alpha-1)}{2\alpha+1}}\) claimed in (\ref{eqn:rate}) since we are in the low-noise regime \(t \lesssim n^{-\frac{2}{2\alpha+1}}\). 

However, it turns out it is not at all necessary for \(\hat{f}(1)\) to be a good estimator of \(f(1)\) in order to achieve good score estimation. First, consider that for any \(\mu \in (-1, 1)\), Taylor expansion around the point \(1\) yields \(f(\mu) = \sum_{k=0}^{\lfloor \alpha \rfloor} \frac{f^{(k)}(1)}{k!} (\mu-1)^k + O(|\mu-1|^{\alpha - \lfloor \alpha \rfloor})\), and so 
\begin{align*}
    (\varphi_t * f)(x) &= \int_{-1}^{1} \varphi_t(x-\mu) f(\mu) \, \rd \mu \\
    &= \sum_{k=0}^{\lfloor \alpha \rfloor} \frac{f^{(k)}(1)}{k!} \int_{-1}^{1} (\mu-1)^k \varphi_t(x - \mu) \, \rd \mu + O\left(\int_{-1}^{1} |\mu-1|^{\alpha} \varphi_t(x-\mu) \, \rd\mu \right). 
\end{align*}
Since \(|x-1| < \sqrt{Ct \log(1/t)}\), it can be shown that the error term is dominated by \((t \log(1/t))^{\alpha/2}\). The same expansion can be applied to \(\varphi_t * \hat{f}\), and so 
\begin{align*}
    &\bE \left(|f(1) (\varphi_t * \hat{f})(x) - \hat{f}(1) (\varphi_t * f)(x)|^2\right) \\
    &\lesssim \bE\left(|f(1)\hat{f}(1) - \hat{f}(1) f(1)|^2\right) \\
    &\;\;\; + \sum_{k=1}^{\lfloor\alpha\rfloor} \frac{\int_{-1}^{1} |\mu-1|^{2k} \varphi_t(x-\mu) \,\rd \mu}{k!} \bE\left(|f(1)\hat{f}^{(k)}(1) - \hat{f}(1)f^{(k)}|^2\right) + (t\log(1/t))^{\alpha} \\
    &\lesssim \sum_{k=1}^{\lfloor \alpha \rfloor} (t\log(1/t))^{k} \cdot n^{-\frac{2(\alpha - k)}{2\alpha+1}} + (t\log(1/t))^{\alpha} \\
    &\lesssim t n^{-\frac{2(\alpha-1)}{2\alpha+1}} \cdot \log^{\alpha}(1/t). 
\end{align*}
Then, since \(\varphi_t(x-1) \lesssim t^{-1/2}\), it follows \(\int_{D_2 \cap \R^+} \bE \left(J_1(x, t)\right) \, \rd x \lesssim n^{-\frac{2(\alpha-1)}{2\alpha+1}} \cdot \sqrt{t} \log^{\alpha+1/2}(1/t) \lesssim n^{-\frac{2(\alpha-1)}{2\alpha+1}}\). The slowdown has been circumvented! The key phenomenon is the cancellation of the first order terms (i.e. corresponding to \(k = 0\)). This extremely convenient cancellation occurs precisely because of the self-normalization in the score function which delivers the nice form of the numerator in (\ref{eqn:intro-2}). No smoothness at all needs to be assumed at the boundary of \(f\)'s support, unlike previous work \cite{oko_diffusion_2023}. 

The analysis of the external part $D_3$ is a simple extension of the analysis of $D_1$ and $D_2$. The only difficulty is to compare the exponential decay rates of the numerator and denominator of (\ref{eqn:intro-2}), but calculations similar to previous ones show the error is still dominated by the errors on \(D_1\) and \(D_2\). Therefore, the following minimax upper bound can be established 
\[\sup_{f \in \mathcal{F}_\alpha} \bE\left(\int_{-\infty}^{\infty} \left|\hat{s}(x, t) - s(x, t)\right|^2 \, p(x, t) \,\rd x \right) \lesssim n^{-\frac{2(\alpha-1)}{2\alpha+1}}.\]

When $\alpha < 1$, the data generating density $f$ need not be differentiable, precluding our earlier arguments which make use of Taylor expansions. In this case, we can show optimal rates can be achieved by using trivial estimators which use no data. Let $\hat{f}(x)=\frac12 \mathbbm{1}_{\{|x|\le 1\}}$ be a trivial density estimator of $f$ and define $\hat{s}(x,t) = \frac{\left(\phi_t'* \hat{f}\right)(x)}{\left(\phi_t* \hat{f}\right)(x)}$. If $0 < \alpha < 1$, it can be shown
\[\sup_{f \in \mathcal{F}_\alpha} \bE\left(\int_{-\infty}^{\infty} \left|\hat{s}(x, t) - s(x, t)\right|^2 \, p(x, t) \,\rd x \right) \lesssim t^{\alpha-1}.\]
Theorem \ref{thm:score_upperbound} follows after combining all of these results. 

==> upper/upper_bound_text.tex <==
For the minimax upper bound for score estimation, we have the following theorem hold for any H\"{o}lder smoothness $\alpha > 0$ and $0 < t \lesssim 1$. 
\begin{theorem}[Main Theorem: Upper Bound]
\label{thm:score_upperbound}
For $\forall \alpha > 0 $, there exists universal constants $c_1 = c_1(\alpha, L) > 0$ and $0 < c_2 = c_2(\alpha, L) \lesssim 1$ only dependent on $\alpha$ and $L$, such that: 
\begin{equation*}
\inf_{\hat{s}} \sup_{f \in \mathcal{F}_\alpha} E\left(\int_{-\infty}^{\infty} \left|\hat{s}(x, t) - s(x, t)\right|^2 \, p(x, t) \,\rd x \right) \le c_1\left(\frac{1}{nt^{3/2}} \wedge \left(n^{-\frac{2(\alpha-1)}{2\alpha+1}} + t^{\alpha-1}\right)\right)
\end{equation*}
holds for $\forall t < c_2$. 
\end{theorem}

As we can see, the score function we are estimating can be written as $s(x,t)=\frac{\psi(x,t)}{p(x,t)} = \frac{\phi_t' \star f(x)}{\phi_t \star f(x)}$ where $\psi(x,t) = \frac{\rd}{\rd x} p(x,t)$ is the density derivative. To start with, a direct idea of constructing a score estimator is to propose unbiased estimators of both the density derivative $\psi(x,t)$ and density $p(x,t)$. Given $n$ i.i.d samples $\mu_1, \mu_2, \ldots, \mu_n \sim f(\mu)$, the unbiased estimators $\hat{\psi}_n(x,t)$ and $\hat{p}_n(x,t)$ can be obtained by replacing $f$ with the empirical distribution $\frac1n\sum_{j=1}^n \delta_{\mu_j}$: 
\[\hat{\psi}_n(x, t) = \frac1n \sum_{j=1}^n \phi_t'(x-\mu_j), ~~~\hat{p}_n(x, t) = \frac1n \sum_{j=1}^n \phi_t(x-\mu_j). \]
Their individual mean integrated squared errors (MISE) only contain the variance terms and can be upper bounded as:
\begin{equation}
\label{eqn:intro-1}
\bE \int_\bR \left|\hat{\psi}_n(x, t) - \psi(x,t)\right|^2 \,\rd x \lesssim \frac{1}{nt^{3/2}}, ~~~\bE \int_\bR \left|\hat{p}_n(x, t) - p(x,t)\right|^2 \,\rd x \lesssim \frac{1}{nt^{1/2}}
\end{equation}
through simple calculation. However, how to upper bound the score estimation error remains a serious problem since the denominator $p(x,t)$ and its estimator $\hat{p}_n(x,t)$ can be exponentially small when $|x|$ is sufficiently large. To overcome this technical obstacle, a regularization trick is widely applied in various existing works [Cite XXX] where the score estimator $\hat{s}_n(x,t) = \frac{\hat{\psi}_n(x,t)}{\hat{p}_n(x,t)\vee \varepsilon}$. Here, $\varepsilon$ is a small constant to prevent the denominator away from 0 and it is usually chosen as $\varepsilon = n^{-2}$. Through regularization by constant, score estimation error can be further controlled by the Hellinger distance, but with additional $\mathrm{polylog} n$ terms required in the upper bound. To avoid those logarithmic terms, we originally apply a function regularizer instead of a constant regularizer, where $\hat{s}_n(x,t) = \frac{\hat{\psi}_n(x,t)}{\hat{p}_n(x,t)\vee \varepsilon(x)}$ with $\varepsilon(x) := c_d\int_{-1}^1 \phi_t(x-\mu) \,\rd \mu $. Notice that $\varepsilon(x) \le p(x,t) \le C_d / c_d \cdot \varepsilon(x)$ always holds, the score estimation error can be split into two individual errors related on density and its derivative as follows:
\begin{equation*}
\bE \left(\hat{s}_n(x,t)-s(x,t)\right)^2\cdot p(x,t) \lesssim \frac{\bE (\hat{\psi}_n(x, t)-\psi(x,t))^2}{p(x,t)} + s(x,t)^2 \cdot \frac{\bE (\hat{p}_n(x, t)-p(x,t))^2}{p(x,t)}.
\end{equation*}
To better understand its integration over $x\in \bR$, we consider three different regions of $x$, the internal part $D_1 = \{x:~|x|<1-\sqrt{Ct\log(1/t)}\}$, the boundary part $D_2 = \{x:~1-\sqrt{Ct\log(1/t)} \le |x| \le 1+C\sqrt{t}\}$ and the external part $D_3 = \{x:~|x| > 1+C\sqrt{t}\}$. When $x\in D_1 \cup D_2$, the density is bounded above from 0 as $p(x,t)\gtrsim 1$ and when $x\in D_1$, the density derivative and score are upper bounded by constants as $\psi(x,t), s(x,t)\lesssim 1$ if the smoothness $\alpha \ge 1$. In the boundary $D_2$, we have $\psi(x,t), s(x,t)\lesssim \frac{1}{\sqrt{t}}$. For the unbiased estimator proposed above, we can easily obtain the integrated bound $\frac{1}{nt^{3/2}}$ when $x\in D_1 \cup D_2$ since $p(x,t)$ is lower bounded by a constant. For the external part $D_3$, we compare the exponential decay rates of the numerator and denominator and show that the score estimation error $\left(\hat{s}_n(x,t)-s(x,t)\right)^2\cdot p(x,t)$ exponentially decays, which leads to a minimax upper bound raised by unbiased estimator:
\[\inf_{\hat{s}} \sup_{f \in \mathcal{F}_\alpha} E\left(\int_{-\infty}^{\infty} \left|\hat{s}(x, t) - s(x, t)\right|^2 \, p(x, t) \,\rd x \right) \lesssim \frac{1}{nt^{3/2}}.\]
The result is far from satisfactory because when the noise level $t\rightarrow 0$, this upper bound goes to infinity. Therefore, we need another estimator with kernel-based estimation of $f$ directly plugged in. Unlike the unbiased estimator, the bound of kernel-based score estimation error is relevant to the smoothness $\alpha$ of the original density $f$. According to [Cite XXX], there exists a kernel-based estimator of $f$, denoted as $\hat{f}$, such that
\[\bE \left(\hat{f}^{(k)}(x) - f^{(k)}(x)\right)^2\lesssim n^{-\frac{2(\alpha-k)}{2\alpha+1}}~~~\forall k=0,1,\ldots, \lfloor\alpha\rfloor\]
holds for $\forall x\in [-1, 1]$. Here, $f^{(k)}$ denotes the $k$-th order derivative of $f$. To construct the score estimator, we directly plug in the kernel-based density estimator $\hat{f}$ and have: $\hat{s}(x,t)=\frac{\left(\phi_t'\star \hat{f}\right)(x)}{\left(\phi_t \star \hat{f}\right)(x)}$. In order to achieve a tight rate, we operate  
\begin{align}
\label{eqn:intro-2}
\hat{s}(x,t)-s(x,t) &=\frac{\left(\phi_t'\star \hat{f}\right)(x)}{\left(\phi_t \star \hat{f}\right)(x)} - \frac{\left(\phi_t'\star f\right)(x)}{\left(\phi_t \star f\right)(x)}\notag \\
&= \frac{\left(\phi_t'\star \hat{f}\right)(x)\cdot\left(\phi_t \star f\right)(x) - \left(\phi_t \star \hat{f}\right)(x)\cdot\left(\phi_t'\star f\right)(x)}{\left(\phi_t \star \hat{f}\right)(x)\cdot \left(\phi_t \star f\right)(x)}. 
\end{align}
instead of splitting the error into the density error and the density derivative error as Equation (\ref{eqn:intro-1}). In the internal part $D_1$, the density derivative error dominates and leads to the $n^{-\frac{2(\alpha-1)}{2\alpha+1}}$ upper bound. For the boundary part $D_2$, it is comprised of the positive and negative halves, as $D_2 = D_2^+ \cup D_2^-$ and the denominator in Equation (\ref{eqn:intro-2}) is lower bounded by constant. When $x\in D_2^+ = D_2 \cap \bR^+$, we know that $|x-1| < \sqrt{Ct\log(1/t)}$ and we take $\lfloor\alpha\rfloor$-th order Taylor expansion of the numerator around $x=1$, again achieving the $n^{-\frac{2(\alpha-1)}{2\alpha+1}}$ upper bound. According to the symmetricity, the same bound holds for the negative half $D_2^-$. The external part $D_3$ is just a simple extension of the upper bounds in $D_1$ and $D_2$. The only difficulty for the external part is to compare the exponential decay rates of the numerator and denominator of Equation (\ref{eqn:intro-2}). Through similar calculation as the unbiased estimator, the external integrated error is still dominated by the internal and boundary integrated errors combined. Therefore, we conclude that the following minimax upper bound raised by kernel-based estimator holds when $\alpha \ge 1$:
\[\inf_{\hat{s}} \sup_{f \in \mathcal{F}_\alpha} E\left(\int_{-\infty}^{\infty} \left|\hat{s}(x, t) - s(x, t)\right|^2 \, p(x, t) \,\rd x \right) \lesssim n^{-\frac{2(\alpha-1)}{2\alpha+1}}.\]
Notice that in the upper bound of kernel-based estimator above, we require the smoothness $\alpha\ge 1$ since our proof is based on Taylor expansion and the integral-by-parts technique:
\[\int_{-1}^1 \phi_t'(x-\mu) f(\mu)\,\rd \mu = \phi_t(x+1)f(-1)-\phi_t(x-1)f(1)+\int_{-1}^1 \phi_t(x-\mu) f'(\mu) \,\rd\mu. \]
However, when $\alpha < 1$, our true density function $f(x)$ is no longer differentiable, which prevents us applying both Taylor expansion and integral-by-parts with $f'(\mu)$ involved. In this case, we have shown that optimal rates can be achieved by using data-free estimators, which means our final bound is independent of sample size $n$. Let $\hat{f}(x)=\frac12 \mathbb I[|x|\le 1]$ to be a trivial density estimator of $f$, we still choose $\hat{s}(x,t) = \frac{\left(\phi_t'\star \hat{f}\right)(x)}{\left(\phi_t\star \hat{f}\right)(x)}$. Through the same proof techniques as kernel-based estimator, we have the following minimax upper bound raised for data-free trivial estimator in the low-smoothness case $0 < \alpha < 1$:
\[\inf_{\hat{s}} \sup_{f \in \mathcal{F}_\alpha} E\left(\int_{-\infty}^{\infty} \left|\hat{s}(x, t) - s(x, t)\right|^2 \, p(x, t) \,\rd x \right) \lesssim t^{\alpha-1}.\]
Finally, we combine our results for unbiased, kernel-based and data-free estimators, which leads to our Theorem \ref{thm:score_upperbound}. 
